Quantitative convergence analysis of iterated expansive, set-valued mappings

We develop a framework for quantitative convergence analysis of Picard iterations of expansive set-valued fixed point mappings. There are two key components of the analysis. The first is a natural generalization of single-valued averaged mappings to expansive, set-valued mappings that characterizes a type of strong calmness of the fixed point mapping. The second component to this analysis is an extension of the well-established notion of metric subregularity -- or inverse calmness -- of the mapping at fixed points. Convergence of expansive fixed point iterations is proved using these two properties, and quantitative estimates are a natural byproduct of the framework. To demonstrate the application of the theory, we prove for the first time a number of results showing local linear convergence of nonconvex cyclic projections for inconsistent (and consistent) feasibility problems, local linear convergence of the forward-backward algorithm for structured optimization without convexity, strong or otherwise, and local linear convergence of the Douglas--Rachford algorithm for structured nonconvex minimization. This theory includes earlier approaches for known results, convex and nonconvex, as special cases.

==> drlmacros.tex <==
%--------------------------
%  PACKAGES
%--------------------------
%
% Autographia packages
\usepackage[utf8]{inputenc}
% \usepackage[francais]{babel}


% SIAM compatible packages:
\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{amssymb}
% \usepackage[pdftex]{graphicx}
% \usepackage{graphicx}
% \usepackage{exscale}
\usepackage{subfigure}
% \usepackage{exscale,relsize}
% \usepackage{fontenc}

% SIAM doesn't like the following:
% \usepackage{calc}
\usepackage{cite}
% \usepackage{mathrsfs}
\usepackage{enumerate}
% \usepackage{changebar}
% \usepackage{pifont}      %needed by dingautolist
\usepackage{fancybox}
% \usepackage{latexsym}

  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % Generates hyperlinked PDF:
\RequirePackage{hyperref}
\PassOptionsToPackage{pdftex,bookmarksopen,bookmarksnumbered}{hyperref}
\voffset=-0.5in
  %
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{hyperref}

% INDEXING COMMANDS
% \usepackage{makeidx}
% \newcommand{\idxdef}[1]{\textbf{\hyperpage{#1}}}
% \newcommand{\idxquo}[1]{\hyperpage{#1}$\dag$}
% \newcommand{\idxfig}[1]{\hyperpage{#1}$\ddag$}

\usepackage[colorinlistoftodos]{todonotes}

%--------------------------
% page settings
%--------------------------
\usepackage{fullpage}
% \usepackage[dvips]{geometry}
% \topmargin 0.0cm
% \oddsidemargin -0.1cm
% \textwidth  16.4cm 
% \headheight 0.0cm
% \textheight 21.7cm
% \parindent  6mm
% \parskip    10pt
% \tolerance  1000

% \usepackage{geometry}
% \geometry{a4paper, left=30mm, right=30mm}
% \topmargin 0.0cm
% \oddsidemargin -0.1cm
% \textwidth  16.4cm 
% \headheight 0.0cm
% \textheight 21.7cm
% \parindent  6mm
% \parskip    10pt
% \tolerance  1000
% \newcommand{\disp}{\displaystyle}
% \newcommand{\betless}{\noalign{\vskip3pt plus 3pt minus 1pt}}
% \newcommand{\bet}{\noalign{\vskip6pt plus 3pt minus 1pt}}
% \newcommand{\betmore}{\noalign{\vskip9pt plus 3pt minus 1pt}}
% \newcommand{\betline}{\noalign{\vskip12pt plus 3pt minus 1pt}}
% \newcommand{\betsp}[1]{\noalign{\vskip#1 plus 3pt minus 1pt}}
% \newcommand{\nn}{\nonumber}
% \newcommand{\alldisp}{\everymath={\displaystyle}}
% \newcommand{\regdisp}{\everymath={\textstyle}}
% \newcommand{\halflongpage}{\enlargethispage{6pt}}
% \newcommand{\onelongpage}{\enlargethispage{12pt}}
% \newcommand{\halfshortpage}{\enlargethispage{-6pt}}
% \newcommand{\oneshortpage}{\enlargethispage{-12pt}}
% \newcommand{\pagebreakeq}{\vskip-\lastskip\pagebreak\ignorespaces\noindent}
% \newcommand{\ununskip}{\vskip-\lastskip}
% \newcommand{\fj}{\linebreak}
% \newcommand{\fjpb}{\vspace*{-\baselineskip}\linebreak} 
% \newcommand{\pfj}{\protect\linebreak} 
% \newcommand{\jamit}{{\spaceskip = .333em plus .167em minus .222em}}
% \newcommand{\ab}{\allowbreak}
% \newcommand{\qqquad}{\qquad\quad}
% \newcommand{\qqqquad}{\qquad\qquad}
% \newcommand{\qm}{\hspace*{\fill}}
% \newcommand{\xf}{\hphantom}
% \newcommand{\bd}{\begin{document}}
% \newcommand{\ed}{\end{document}}
% \newcommand{\clearabove}{\rule{0pt}{9pt}}
% \newcommand{\clearbelow}{\rule[-5pt]{0pt}{9pt}}
% \newcommand{\clearboth}{\rule[-5pt]{0pt}{14pt}}
% \newcommand{\spaceouttable}{\renewcommand{\arraystretch}{1.2}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  Graphics
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{pstricks}
\usepackage{pst-plot}
%\usepackage{pst-3dplot}
\usepackage{pstricks-add}
\usepackage{color}
% \usepackage[doc]{optional}
% \usepackage{float}
% \usepackage{soul}
% \usepackage{graphicx}
% \usepackage{lmodern,bm}
% \usepackage{arcs}

%%%%%%%%%%%%%%%%

\definecolor{labelkey}{rgb}{0,0.08,0.45}
\definecolor{refkey}{rgb}{0,0.6,0.0}
\definecolor{Brown}{rgb}{0.45,0.0,0.05}
\definecolor{lime}{rgb}{0.00,0.8,0.0}
\definecolor{lblue}{rgb}{0.5,0.5,0.99}
\definecolor{lblue}{rgb}{0.8,0.85,1.00}
\definecolor{anotherblue}{rgb}{.8, .8,1}
\definecolor{violet}{rgb}{0.9,0.6,0.9}
\definecolor{greenyellow}{rgb}{0.53,0.99,0.18}
\definecolor{Lyellow}{rgb}{0.99,0.99,0.87}
\definecolor{Lgray}{rgb}{0.93,0.93,0.93}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Boxes
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{rotating}
\usepackage{graphicx}
\usepackage{graphics}
\usepackage{longtable}
\usepackage{fancybox}

\newcommand{\boxedeqn}[1]{%
    \[\fbox{%
        \addtolength{\linewidth}{-2\fboxsep}%
        \addtolength{\linewidth}{-2\fboxrule}%
        \begin{minipage}{\linewidth}%
        \[#1\\[+4mm]\]%
        \end{minipage}%
      }\]%
  }
\newcommand{\boxedtxt}[1]{%
    \[\fbox{%
        \addtolength{\linewidth}{-2\fboxsep}%
        \addtolength{\linewidth}{-2\fboxrule}%
        \begin{minipage}{\linewidth}%
        #1\\[+4mm]%
        \end{minipage}%
      }\]%
  }

%--------------------------
%  MACROS
%--------------------------
%
% Theorems
%
% \usepackage{theorem} % SIAM does not like
\usepackage{amsthm} % SIAM does not like
\newtheorem{thm}{Theorem}[section]
% \newtheorem{theorem}{Theorem}[section]
\newtheorem{fact}[thm]{Fact}
\newtheorem{lemma}[thm]{Lemma}
\newtheorem{proposition}[thm]{Proposition}
\newtheorem{cor}[thm]{Corollary}
\newtheorem{corollary}[thm]{Corollary}
\newtheorem{propn}[thm]{Proposition}
% \newtheorem{definition}[theorem]{Definition}
\newtheorem{defn}[thm]{Definition}
\newtheorem{definition}[thm]{Definition}
% \theoremstyle{plain}{\theorembodyfont{\rmfamily}%
\newtheorem{assumption}[thm]{Assumption}
\newtheorem{condition}[thm]{Condition}
\newtheorem{conjecture}[thm]{Conjecture}
% \theoremstyle{plain}{\theorembodyfont{\rmfamily}% use with {theorem} package
\newtheorem{alg}[thm]{Algorithm}
% \theoremstyle{plain}{\theorembodyfont{\rmfamily}%
% \newtheorem{algorithm}[thm]{Algorithm}
% \theoremstyle{plain}{\theorembodyfont{\rmfamily}%
\newtheorem{eg}[thm]{Example}
\newtheorem{ex}[thm]{Exercise}
% \theoremstyle{plain}{\theorembodyfont{\rmfamily}%
\newtheorem{remark}[thm]{Remark}
% \theoremstyle{plain}{\theorembodyfont{\rmfamily}%
\def\proof{\noindent{\it Proof}. \ignorespaces}
\def\endproof{\vbox{\hrule height0.6pt\hbox{\vrule height1.3ex%
width0.6pt\hskip0.8ex\vrule width0.6pt}\hrule height0.6pt}\medskip}
\def\proofsketch{\noindent{\it Proof sketch}. \ignorespaces}
\def\endproofsketch{\vbox{\hrule height0.6pt\hbox{\vrule height1.3ex%
width0.6pt\hskip0.8ex\vrule width0.6pt}\hrule height0.6pt}\medskip}
\def\detail{\noindent{\it Detail}. \ignorespaces}
\def\enddetail{\vbox{\hrule height0.6pt\hbox{\vrule height1.3ex%
width0.6pt\hskip0.8ex\vrule width0.6pt}\hrule height0.6pt}\medskip}
\renewcommand{\labelenumi}{\rm (\arabic{enumi})}
\renewcommand{\labelenumii}{\rm (\alph{enumii})}
% \numberwithin{equation}{section}
% reference:
\newcommand{\eqr}[1]{Eq.(\ref{#1})}
\newcommand{\figr}[1]{Figure \ref{#1}}

% %Detailed calculations not meant for publication:
% \newcommand{\detail}[1]{\par\noi{\bf [Proof detail\ }{#1}
% \hfill{\bf ]}\par\noi\hspace{-4pt}}
% \renewcommand{\detail}[1]{}
% 
% 
% use as
% 
% \detail{ text }
% 
% lines:
% \rule[4pt]{6.8in}{0.05cm}\\


%-------------------------------
% Fonts and accents
%-------------------------------
%
% caligraphic:
\newcommand{\Acal}{{\mathcal A}}
\newcommand{\Bcal}{{\mathcal B}}
\newcommand{\Ccal}{{\mathcal C}}
\newcommand{\Dcal}{{\mathcal D}}
\newcommand{\Ecal}{{\mathcal E}}
\newcommand{\Fcal}{{\mathcal F}}
\newcommand{\Gcal}{{\mathcal G}}
\newcommand{\Hcal}{{\mathcal H}}
\newcommand{\Ical}{{\mathcal I}}
\newcommand{\Jcal}{{\mathcal J}}
\newcommand{\Kcal}{{\mathcal K}}
\newcommand{\Lcal}{{\mathcal L}}
\newcommand{\Mcal}{{\mathcal M}}
\newcommand{\Ncal}{{\mathcal N}}
\newcommand{\Ocal}{{\mathcal O}}
\newcommand{\Pcal}{{\mathcal P}}
\newcommand{\Qcal}{{\mathcal Q}}
\newcommand{\Rcal}{{\mathcal R}}
\newcommand{\Scal}{{\mathcal S}}
\newcommand{\Tcal}{{\mathcal T}}
\newcommand{\Ucal}{{\mathcal U}}
\newcommand{\Vcal}{{\mathcal V}}
\newcommand{\Wcal}{{\mathcal W}}
\newcommand{\Ycal}{{\mathcal Y}}
\newcommand{\Xcal}{{\mathcal X}}
\newcommand{\Zcal}{{\mathcal Z}}
\newcommand{\acal}{{\mathcal a}}

% mathbb
\newcommand{\Abb}{\mathbb{A}}
\renewcommand{\Bbb}{\mathbb{B}}
\newcommand{\Cbb}{\mathbb{C}}
\newcommand{\Dbb}{\mathbb{D}}
\newcommand{\Ebb}{\mathbb{E}}
\newcommand{\Fbb}{\mathbb{F}}
\newcommand{\Gbb}{\mathbb{G}}
\newcommand{\Hbb}{\mathbb{H}}
\newcommand{\Ibb}{\mathbb{I}}
\newcommand{\Jbb}{\mathbb{J}}
\newcommand{\Kbb}{\mathbb{K}}
\newcommand{\Mbb}{\mathbb{M}}
\newcommand{\Nbb}{\mathbb{N}}
\newcommand{\Obb}{\mathbb{O}}
\newcommand{\Pbb}{\mathbb{P}}
\newcommand{\Qbb}{\mathbb{Q}}
\newcommand{\Rbb}{\mathbb{R}}
\newcommand{\Sbb}{\mathbb{S}}
\newcommand{\Tbb}{\mathbb{T}}
\newcommand{\Ubb}{\mathbb{U}}
\newcommand{\Vbb}{\mathbb{V}}
\newcommand{\Wbb}{\mathbb{W}}
\newcommand{\Xbb}{\mathbb{X}}
\newcommand{\Ybb}{\mathbb{Y}}
\newcommand{\Zbb}{\mathbb{Z}}

% hats
\newcommand{\Ahat}{{\widehat{A}}}
\newcommand{\Bhat}{{\widehat{B}}}
\newcommand{\Chat}{{\widehat{C}}}
\newcommand{\Dhat}{{\widehat{D}}}
\newcommand{\Ehat}{{\widehat{E}}}
\newcommand{\Fhat}{{\widehat{F}}}
\newcommand{\Ghat}{{\widehat{G}}}
\newcommand{\Hhat}{{\widehat{H}}}
\newcommand{\Ihat}{{\widehat{I}}}
\newcommand{\Jhat}{{\widehat{J}}}
\newcommand{\Khat}{{\widehat{K}}}
\newcommand{\Lhat}{{\widehat{L}}}
\newcommand{\Mhat}{{\widehat{M}}}
\newcommand{\Nhat}{{\widehat{N}}}
\newcommand{\Phat}{{\widehat{P}}}
\newcommand{\Qhat}{{\widehat{Q}}}
\newcommand{\Rhat}{{\widehat{R}}}
\newcommand{\Shat}{{\widehat{S}}}
\newcommand{\That}{{\widehat{T}}}
\newcommand{\Uhat}{{\widehat{U}}}
\newcommand{\Vhat}{{\widehat{V}}}
\newcommand{\What}{{\widehat{W}}}
\newcommand{\Xhat}{{\widehat{X}}}
\newcommand{\Yhat}{{\widehat{Y}}}
\newcommand{\Zhat}{{\widehat{Z}}}
\newcommand{\ahat}{{\widehat{a}}}
\newcommand{\bhat}{{\widehat{b}}}
\newcommand{\chat}{{\widehat{c}}}
\newcommand{\dhat}{{\widehat{d}}}
\newcommand{\ehat}{{\widehat{e}}}
\newcommand{\fhat}{{\widehat{f}}}
\newcommand{\ghat}{{\widehat{g}}}
\newcommand{\hhat}{{\widehat{h}}}
\newcommand{\ihat}{{\widehat{i}}}
\newcommand{\jhat}{{\widehat{j}}}
\newcommand{\khat}{{\widehat{k}}}
\newcommand{\lhat}{{\widehat{l}}}
\newcommand{\mhat}{{\widehat{m}}}
\newcommand{\nhat}{{\widehat{n}}}
\newcommand{\phat}{{\widehat{p}}}
\newcommand{\qhat}{{\widehat{q}}}
\newcommand{\rhat}{{\widehat{r}}}
\newcommand{\shat}{{\widehat{s}}}
\newcommand{\that}{{\widehat{t}}}
\newcommand{\uhat}{{\widehat{u}}}
\newcommand{\vhat}{{\widehat{v}}}
\newcommand{\what}{{\widehat{w}}}
\newcommand{\xhat}{{\widehat{x}}}
\newcommand{\yhat}{{\widehat{y}}}
\newcommand{\zhat}{{\widehat{z}}}

\newcommand{\alphahat}{{\widehat{\alpha}}}
\newcommand{\betahat}{{\widehat{\beta}}}
\newcommand{\epsilonhat}{{\widehat{\epsilon}}}
\newcommand{\gammahat}{{\widehat{\gamma}}}
\newcommand{\deltahat}{{\widehat{\delta}}}
\newcommand{\etahat}{{\widehat{\eta}}}
\newcommand{\kappahat}{{\widehat{\kappa}}}
\newcommand{\phihat}{{\widehat{\phi}}}
\newcommand{\psihat}{{\widehat{\psi}}}
\newcommand{\sigmahat}{{\widehat{\sigma}}}
\newcommand{\Omegahat}{{\widehat{\Omega}}}
\newcommand{\omegahat}{{\widehat{\omega}}}
\newcommand{\rhohat}{{\widehat{\rho}}}
\newcommand{\zetahat}{{\widehat{\zeta}}}

% bars
\newcommand{\Abar}{{\overline{A}}}
\newcommand{\Bbar}{{\overline{B}}}
\newcommand{\Cbar}{{\overline{C}}}
\newcommand{\Dbar}{{\overline{D}}}
\newcommand{\Ebar}{{\overline{E}}}
\newcommand{\Fbar}{{\overline{F}}}
\newcommand{\Gbar}{{\overline{G}}}
\newcommand{\Hbar}{{\overline{H}}}
\newcommand{\Ibar}{{\overline{I}}}
\newcommand{\Jbar}{{\overline{J}}}
\newcommand{\Kbar}{{\overline{K}}}
\newcommand{\Lbar}{{\overline{L}}}
\newcommand{\Mbar}{{\overline{M}}}
\newcommand{\Nbar}{{\overline{N}}}
\newcommand{\Pbar}{{\overline{P}}}
\newcommand{\Qbar}{{\overline{Q}}}
\newcommand{\Rbar}{{\overline{R}}}
\newcommand{\Sbar}{{\overline{S}}}
\newcommand{\Tbar}{{\overline{T}}}
\newcommand{\Ubar}{{\overline{U}}}
\newcommand{\Vbar}{{\overline{V}}}
\newcommand{\Wbar}{{\overline{W}}}
\newcommand{\Xbar}{{\overline{X}}}
\newcommand{\Ybar}{{\overline{Y}}}
\newcommand{\Zbar}{{\overline{Z}}}
\newcommand{\abar}{{\overline{a}}}
\newcommand{\bbar}{{\overline{b}}}
\newcommand{\cbar}{{\overline{c}}}
\newcommand{\dbar}{{\overline{d}}}
\newcommand{\ebar}{{\overline{e}}}
\newcommand{\fbar}{{\overline{f}}}
\newcommand{\gbar}{{\overline{g}}}
% \newcommand{\hbar}{{\overline{h}}}
\newcommand{\ibar}{{\overline{i}}}
\newcommand{\jbar}{{\overline{j}}}
\newcommand{\kbar}{{\overline{k}}}
\newcommand{\lbar}{{\overline{l}}}
\newcommand{\mbar}{{\overline{m}}}
\newcommand{\nbar}{{\overline{n}}}
\newcommand{\pbar}{{\overline{p}}}
\newcommand{\qbar}{{\overline{q}}}
\newcommand{\rbar}{{\overline{r}}}
\newcommand{\sbar}{{\overline{s}}}
\newcommand{\tbar}{{\overline{t}}}
\newcommand{\ubar}{{\overline{u}}}
\newcommand{\vbar}{{\overline{v}}}
\newcommand{\wbar}{{\overline{w}}}
\newcommand{\xbar}{{\overline{x}}}
\newcommand{\ybar}{{\overline{y}}}
\newcommand{\zbar}{{\overline{z}}}

\newcommand{\alphabar}{{\overline{\alpha}}}
\newcommand{\betabar}{{\overline{\beta}}}
\newcommand{\nubar}{{\overline{\nu}}}
\newcommand{\mubar}{{\overline{\mu}}}
\newcommand{\gammabar}{{\overline{\gamma}}}
\newcommand{\epsilonbar}{{\overline{\epsilon}}}
\newcommand{\varepsilonbar}{{\overline{\varepsilon}}}
\newcommand{\deltabar}{{\overline{\delta}}}
\newcommand{\etabar}{{\overline{\eta}}}
\newcommand{\kappabar}{{\overline{\kappa}}}
\newcommand{\lambdabar}{{\overline{\lambda}}}
\newcommand{\phibar}{{\overline{\phi}}}
\newcommand{\psibar}{{\overline{\psi}}}
\newcommand{\rhobar}{{\overline{\rho}}}
\newcommand{\thetabar}{{\overline{\theta}}}
\newcommand{\zetabar}{{\overline{\zeta}}}
\newcommand{\Omegabar}{{\overline{\Omega}}}

% tildes
\newcommand{\Atilde}{{\widetilde{A}}}
\newcommand{\Btilde}{{\widetilde{B}}}
\newcommand{\Ctilde}{{\widetilde{C}}}
\newcommand{\Dtilde}{{\widetilde{D}}}
\newcommand{\Etilde}{{\widetilde{E}}}
\newcommand{\Ftilde}{{\widetilde{F}}}
\newcommand{\Gtilde}{{\widetilde{G}}}
\newcommand{\Htilde}{{\widetilde{H}}}
\newcommand{\Itilde}{{\widetilde{I}}}
\newcommand{\Jtilde}{{\widetilde{J}}}
\newcommand{\Ktilde}{{\widetilde{K}}}
\newcommand{\Ltilde}{{\widetilde{L}}}
\newcommand{\Mtilde}{{\widetilde{M}}}
\newcommand{\Ntilde}{{\widetilde{N}}}
\newcommand{\Ptilde}{{\widetilde{P}}}
\newcommand{\Qtilde}{{\widetilde{Q}}}
\newcommand{\Rtilde}{{\widetilde{R}}}
\newcommand{\Stilde}{{\widetilde{S}}}
\newcommand{\Ttilde}{{\widetilde{T}}}
\newcommand{\Utilde}{{\widetilde{U}}}
\newcommand{\Vtilde}{{\widetilde{V}}}
\newcommand{\Wtilde}{{\widetilde{W}}}
\newcommand{\Xtilde}{{\widetilde{X}}}
\newcommand{\Ytilde}{{\widetilde{Y}}}
\newcommand{\Ztilde}{{\widetilde{Z}}}
\newcommand{\atilde}{{\widetilde{a}}}
\newcommand{\btilde}{{\widetilde{b}}}
\newcommand{\ctilde}{{\widetilde{c}}}
\newcommand{\dtilde}{{\widetilde{d}}}
\newcommand{\etilde}{{\widetilde{e}}}
\newcommand{\ftilde}{{\widetilde{f}}}
\newcommand{\gtilde}{{\widetilde{g}}}
\newcommand{\htilde}{{\widetilde{h}}}
\newcommand{\itilde}{{\widetilde{i}}}
\newcommand{\jtilde}{{\widetilde{j}}}
\newcommand{\ktilde}{{\widetilde{k}}}
\newcommand{\ltilde}{{\widetilde{l}}}
\newcommand{\mtilde}{{\widetilde{m}}}
\newcommand{\ntilde}{{\widetilde{n}}}
\newcommand{\ptilde}{{\widetilde{p}}}
\newcommand{\qtilde}{{\widetilde{q}}}
\newcommand{\rtilde}{{\widetilde{r}}}
\newcommand{\stilde}{{\widetilde{s}}}
\newcommand{\ttilde}{{\widetilde{t}}}
\newcommand{\utilde}{{\widetilde{u}}}
\newcommand{\vtilde}{{\widetilde{v}}}
\newcommand{\wtilde}{{\widetilde{w}}}
\newcommand{\xtilde}{{\widetilde{x}}}
\newcommand{\ytilde}{{\widetilde{y}}}
\newcommand{\ztilde}{{\widetilde{z}}}

\newcommand{\alphatilde}{{\widetilde{\alpha}}}
\newcommand{\betatilde}{{\widetilde{\beta}}}
\newcommand{\epsilontilde}{{\widetilde{\epsilon}}}
\newcommand{\varepsilontilde}{{\widetilde{\varepsilon}}}
\newcommand{\gammatilde}{{\widetilde{\gamma}}}
\newcommand{\deltatilde}{{\widetilde{\delta}}}
\newcommand{\etatilde}{{\widetilde{\eta}}}
\newcommand{\kappatilde}{{\widetilde{\kappa}}}
\newcommand{\phitilde}{{\widetilde{\phi}}}
\newcommand{\psitilde}{{\widetilde{\psi}}}
\newcommand{\zetatilde}{{\widetilde{\zeta}}}
\newcommand{\Omegatilde}{{\widetilde{\Omega}}}
\newcommand{\Psitilde}{{\widetilde{\Psi}}}
\newcommand{\Phitilde}{{\widetilde{\Phi}}}

% boldface
\newcommand{\Abf}{{\bf{A}}}
\newcommand{\Bbf}{{\bf{B}}}
\newcommand{\Cbf}{{\bf{C}}}
\newcommand{\Dbf}{{\bf{D}}}
\newcommand{\Ebf}{{\bf{E}}}
\newcommand{\Fbf}{{\bf{F}}}
\newcommand{\Gbf}{{\bf{G}}}
\newcommand{\Hbf}{{\bf{H}}}
\newcommand{\Ibf}{{\bf{I}}}
\newcommand{\Jbf}{{\bf{J}}}
\newcommand{\Kbf}{{\bf{K}}}
\newcommand{\Lbf}{{\bf{L}}}
\newcommand{\Mbf}{{\bf{M}}}
\newcommand{\Nbf}{{\bf{N}}}
\newcommand{\Pbf}{{\bf{P}}}
\newcommand{\Qbf}{{\bf{Q}}}
\newcommand{\Rbf}{{\bf{R}}}
\newcommand{\Sbf}{{\bf{S}}}
\newcommand{\Tbf}{{\bf{T}}}
\newcommand{\Ubf}{{\bf{U}}}
\newcommand{\Vbf}{{\bf{V}}}
\newcommand{\Wbf}{{\bf{W}}}
\newcommand{\Xbf}{{\bf{X}}}
\newcommand{\Ybf}{{\bf{Y}}}
\newcommand{\Zbf}{{\bf{Z}}}
\newcommand{\abf}{{\bf{a}}}
\newcommand{\bbf}{{\bf{b}}}
\newcommand{\cbf}{{\bf{c}}}
\newcommand{\dbf}{{\bf{d}}}
\newcommand{\ebf}{{\bf{e}}}
\newcommand{\fbf}{{\bf{f}}}
\newcommand{\gbf}{{\bf{g}}}
% \newcommand{\hbf}{{\bf{h}}}
\newcommand{\ibf}{{\bf{i}}}
\newcommand{\jbf}{{\bf{j}}}
\newcommand{\kbf}{{\bf{k}}}
\newcommand{\lbf}{{\bf{l}}}
\newcommand{\mbf}{{\bf{m}}}
\newcommand{\nbf}{{\bf{n}}}
\newcommand{\pbf}{{\bf{p}}}
\newcommand{\qbf}{{\bf{q}}}
\newcommand{\rbf}{{\bf{r}}}
\newcommand{\sbf}{{\bf{s}}}
\newcommand{\tbf}{{\bf{t}}}
\newcommand{\ubf}{{\bf{u}}}
\newcommand{\vbf}{{\bf{v}}}
\newcommand{\wbf}{{\bf{w}}}
\newcommand{\xbf}{{\bf{x}}}
\newcommand{\ybf}{{\bf{y}}}
\newcommand{\zbf}{{\bf{z}}}

\newcommand{\alphabf}{{\bf{\alpha}}}
\newcommand{\betabf}{{\bf{\beta}}}
\newcommand{\nubf}{{\bf{\nu}}}
\newcommand{\gammabf}{{\bf{\gamma}}}
\newcommand{\deltabf}{{\bf{\delta}}}
\newcommand{\etabf}{{\bf{\eta}}}
\newcommand{\kappabf}{{\bf{\kappa}}}
\newcommand{\lambdabf}{{\bf{\lambda}}}
\newcommand{\phibf}{{\bf{\phi}}}
\newcommand{\Phibf}{{\bf{\Phi}}}
\newcommand{\psibf}{{\bf{\psi}}}
\newcommand{\zetabf}{{\bf{\zeta}}}
\newcommand{\Omegabf}{{\bf{\Omega}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% oft used constructs and miscellany:
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% General:
\newcommand{\Hilbert}{\mathcal{H}}
\newcommand{\Euclid}{\mathbb{E}}
\newcommand{\setto}{\rightrightarrows}
\newcommand{\paren}[1]{\left(#1\right)}
\newcommand{\ecklam}[1]{\left[#1\right]}
\newcommand{\klam}[1]{\left\{#1\right\}}
\newcommand{\veps}{\varepsilon}
\def\Upon#1#2{ {{\displaystyle #1}\over {\displaystyle #2}} }
\renewcommand{\Im}{{\rm Im}}
\renewcommand{\Re}{{\rm Re}}
\renewcommand{\equiv}{:=}
\newcommand{\cint}{\circ\!\!\!\!\!\int}
\newcommand{\toinf}{\rightarrow\infty}
\newcommand{\pinf}{+\infty}
\newcommand{\tozero}{\rightarrow 0}
\newcommand{\attains}[1]{\rightarrow_{\!\!\!\!\!\!\!{_#1}}~}
\newcommand{\emp}{\ensuremath{\text{{\sffamily\O}}}}
\newcommand{\Ball}{{\Bbb}}
% \newcommand{\ball}{{\Bbb}}
\newcommand{\ball}[2]{\Ball_{#2}\left({#1}\right)}
\newcommand{\Rn}{{\Rbb^n}}
\newcommand{\Cn}{{\Cbb^n}}
\newcommand{\Rnp}{{\Rbb^n_+}}
\newcommand{\Rnn}{{\Rbb^{n\times n}}}
\newcommand{\Rmn}{{\Rbb^{m\times n}}}
\newcommand{\Rm}{{\Rbb^m}}
\newcommand{\Rk}{{\Rbb^k}}
\newcommand{\Rp}{{\Rbb_+}}
\newcommand{\Rpp}{{\Rbb_{++}}}
\newcommand{\Rth}{{\Rbb^3}}
\newcommand{\Rtw}{{\Rbb^2}}
\newcommand{\extre}{(-\infty,+\infty]}
\newcommand{\extrem}{[-\infty,+\infty]}
\newcommand{\cc}[1]{\overline{#1}}
\newcommand{\ucmin}[2]{\underset{#2}{\mbox{minimize}}~#1}
\newcommand{\argucmin}[2]{\underset{#2}{\mbox{argmin}}~#1}
\newcommand{\cmin}[3]{\begin{array}{ll}\underset{#2}{\mbox{minimize }}\qquad #1&\\
                       \mbox{subject to }\qquad#3&\end{array}}

\newcommand{\ucmax}[2]{\underset{#2}{\mbox{maximize}}~#1}
\newcommand{\cmax}[3]{\begin{array}{ll}\underset{#2}{\mbox{maximize }}\qquad #1&\\
                       \mbox{subject to }\qquad#3&\end{array}}
\newcommand{\set}[2]{\left\{#1\,\left|\,#2\right.\right\}}
\newcommand{\map}[3]{#1:\,#2\rightarrow #3\,}
\newcommand{\mmap}[3]{#1:\,#2\rightrightarrows #3\,}
\newcommand{\pd}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\pdd}[2]{\frac{\partial^2 #1}{\partial #2^2}}
\newcommand{\pdn}[2]{\frac{\partial^n #1}{\partial #2^n}}
% \newcommand{\D}[2]{\frac{d #1}{d #2}}
\newcommand{\DD}[2]{\frac{d^2 #1}{d #2^2}}
\newcommand{\Dn}[2]{\frac{d^n #1}{d #2^n}}

\newcommand{\vect}[1]{{\boldsymbol #1}}
\newcommand{\ip}[2]{\left\langle #1,~ #2\right\rangle}
\newcommand{\twxo}[2]{\left(\begin{array}{c}#1 \\#2\end{array}\right)}
\newcommand{\thxo}[3]{\left(\begin{array}{c}#1 \\#2\\#3\end{array}\right)}
\newcommand{\thxth}[9]{\left(\begin{array}{ccc}#1 &#2&#3\\#4 &#5&#6\\#7 &#8&#9\end{array}\right)}
\newcommand{\twxtw}[4]{\left(\begin{array}{cc}#1 &#2\\#3&#4\end{array}\right)}
\newcommand{\normsq}[1]{\left\|#1\right\|^2}
\newcommand{\norm}[1]{\left\|#1\right\|}
\newcommand{\norminf}[1]{\left\|#1\right\|_{\infty}}
\newcommand{\itr}[2]{{#1^{{#2}}}}
\newcommand{\seq}[1]{{\left(\itr{#1}{k}\right)_{k\in\Nbb}}}

\newcommand{\compl}[1]{#1^{\circ}}
\renewcommand{\choose}[2]{\left(\begin{array}{c}\!#1\!\\\!#2\!\end{array}\right)}
\newcommand{\modu}{\!\!\!\!\!\mod\!}
\newcommand{\as}{\qquad\mbox{a.s.}}
\newcommand{\asto}{\overset{a.s.}{\to}}
\newcommand{\im}{{\rm {\scriptstyle i}}}
\newcommand{\und}{\quad\mbox{and}\quad}
\newcommand{\where}{\quad\mbox{ where }\quad}
\newcommand{\fur}{\mbox{ for }}
\newcommand{\ow}{\mbox{ otherwise }}
\newcommand{\spcl}[1]{{{#1}_*}}
% \newcommand{\qed}{\hfill $\Box$ \\ \medskip}

% Variational Analysis:
\DeclareMathOperator{\atan}{atan}
\DeclareMathOperator{\Id}{Id}
\DeclareMathOperator{\id}{Id}
\DeclareMathOperator{\diverg}{div}
\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\prox}{prox}
\DeclareMathOperator{\limi}{\varliminf}
\DeclareMathOperator{\lims}{\varlimsup}
\DeclareMathOperator{\elims}{e-\limsup}
\DeclareMathOperator{\elimi}{e-\liminf}
\DeclareMathOperator{\elim}{e-\lim}
\DeclareMathOperator{\plims}{p-\limsup}
\DeclareMathOperator{\plimi}{p-\liminf}
\DeclareMathOperator{\plim}{p-\lim}
\DeclareMathOperator{\glims}{g-\limsup}
\DeclareMathOperator{\glimi}{g-\liminf}
\DeclareMathOperator{\glim}{g-\lim}
\DeclareMathOperator{\hzn}{hzn}
\DeclareMathOperator{\csm}{csm}
\DeclareMathOperator{\weakly}{\rightharpoonup}
\DeclareMathOperator{\weakstarly}{\stackrel{\mathrm{w*}}{\rightharpoondown}}
\DeclareMathOperator{\xtoinf}{\|\text{$x$}\| \rightarrow +\infty}
\DeclareMathOperator{\sgn}{sign\,}
\DeclareMathOperator{\sinc}{sinc\,}
\DeclareMathOperator{\argmax}{argmax\,}
\DeclareMathOperator{\argmin}{argmin\,}
\DeclareMathOperator{\eargmin}{\text{$\varepsilon$}-argmin\,}
\DeclareMathOperator{\dist}{dist}
\DeclareMathOperator{\kernel}{null\,}
\DeclareMathOperator{\dir}{dir\,}
\DeclareMathOperator{\lev}{{lev\,}}
\DeclareMathOperator{\bdy}{{bdy\,}}
% \newcommand{\bdy}{\partial}
\DeclareMathOperator{\cone}{{cone}}
\newcommand{\ccone}{\ensuremath{\overline{\operatorname{cone}}\,}}
\DeclareMathOperator{\dom}{{dom\,}}
\DeclareMathOperator{\gph}{gph}
\newcommand{\pa}{\ensuremath{\operatorname{par}}}
\DeclareMathOperator{\Supp}{supp} % siam doesn't like this
\DeclareMathOperator{\conv}{conv}
\newcommand{\cconv}{\ensuremath{\overline{\operatorname{conv}}\,}}
\DeclareMathOperator{\hull}{co\,}
\DeclareMathOperator{\aff}{aff}
\DeclareMathOperator{\intr}{int\,}
\DeclareMathOperator{\cont}{cont\,}
\DeclareMathOperator{\core}{core\,}
\DeclareMathOperator{\trace}{{\bf Tr}\,}
\DeclareMathOperator{\mdiag}{diag\,} % siam doesn't like this
\DeclareMathOperator{\vdiag}{Diag\,} % siam doesn't like this
\DeclareMathOperator{\Fix}{\mathsf{Fix}\,}
% \DeclareMathOperator*{\Fix}{Fix} %Set of fixed points
\DeclareMathOperator{\Find}{\mathsf{Find}\,}
\DeclareMathOperator{\range}{{\rm range}}
\DeclareMathOperator{\rank}{{\rm rank}}
\DeclareMathOperator{\Span}{{\rm span}}
\newcommand{\card}{\ensuremath{\operatorname{card}}}
\newcommand{\lspan}{\ensuremath{\operatorname{span}}}
% \renewcommand{\span}{\ensuremath{\rm span}}
\DeclareMathOperator{\epi}{{\rm epi}}
% \newcommand{\epi}[1]{{\mbox{epi}\, #1}}
\DeclareMathOperator{\sepi}{{\scriptsize epi}}
% \newcommand{\sepi}[1]{{\mbox{\scriptsize epi}\, (#1)}}
\newcommand{\tcone}[1]{{T}_{#1}}
\newcommand{\ncone}[1]{{N}_{#1}}
\newcommand{\encone}[1]{{\widehat{N}}^\epsilon_{#1}}
\newcommand{\fncone}[1]{{\widehat{N}}_{#1}}
% \newcommand{\fncone}[1]{N^{\text{\rm Fr\'e}}_{#1}}
\newcommand{\pncone}[1]{N^{\text{\rm prox}}_{#1}} %proximal normal cone
\newcommand{\rpncone}[2]{N^{\text{\rm prox}}_{#1|#2}} %restricetd proximal 
\newcommand{\rncone}[2]{N_{#1|#2}} %restricetd normal cone 

\newcommand{\cl}{\mbox{\rm cl}\,}
\newcommand{\wstcl}[1]{{\mbox{{\rm cl}}^*\left( #1\right)}}
\newcommand{\wcl}{{\mbox{cl}^*\,}}
\newcommand{\closu}[1]{\ensuremath{\overline{#1}}}
% \newcommand{\intr}[1]{{\mbox{int}\;#1}}
% \newcommand{\ri}[1]{{\mbox{ri}\;#1}}
\newcommand{\reli}{\ensuremath{\operatorname{ri}}}
\newcommand{\polar}[1]{{\left( #1\right)^\circ}}
\newcommand{\support}[1]{{\psi^*_{#1}}}
\newcommand{\sd}{\partial}
\newcommand{\sdinf}{\partial^\infty}
\newcommand{\csd}{{\overline\partial}}
\newcommand{\rsd}{{\widehat\partial}}
\newcommand{\fsd}{{\widehat\partial}}
% \newcommand{\fsd}{{\partial^{\text{\rm Fr\'e}}}}
\newcommand{\rsg}{{\widehat d}}


% Scattering:
\newcommand{\uinf}{u^{\infty}}
\newcommand{\us}{u^{s}}
\newcommand{\ui}{u^{i}}
\newcommand{\winf}{w^{\infty}}
\newcommand{\ws}{w^{s}}
\newcommand{\wi}{w^{i}}
\newcommand{\vinf}{v^{\infty}}
\newcommand{\vs}{v^{s}}
\newcommand{\vi}{v^{i}}
\newcommand{\ps}{\Phi}             % point source
\newcommand{\psinf}{\Phi{^\infty}}  % far field pattern of point source
\newcommand{\di}{\etahat}              % incident field direction
\newcommand{\scd}{\Omega}                           % scattering domain (assumed closed)
\newcommand{\oexter}{\scd^o}   % open exterior of scattering domain
\newcommand{\exter}{\cl{\scd^o}}   % open exterior of scattering domain
\newcommand{\bdyint}[1]{\int_{\!\bdy #1}}

%
%=========================================
%    End macros
%=========================================


